The Gaia Ultracool Dwarf Sample -- V: The Ultracool Dwarf Companion catalogue

We present the Ultracool Dwarf Companion Catalogue of 278 multiple systems, 32 of which are newly discovered, each with at least one spectroscopically confirmed Ultracool Dwarf, within a 100 pc volume-limited sample. This catalogue is compiled using the Gaia Catalogue of Nearby Stars for stellar primaries and the Gaia Ultracool Dwarf Sample for low-mass companions and includes 241 doubles, 33 triples, and 4 higher-order systems established from positional, proper motion, and parallax constraints. The catalogue seeks to identify probable benchmark systems within 100 pc to obtain model-independent astrophysical parameters of Ultracool Dwarfs. Chance alignment probabilities are calculated to evaluate the physical nature of each system. Astrometric and photometric data from Gaia Data Release 3 and the Two Micron All Sky Survey are included for all objects. We identify potential unseen companions using a combination of the Renormalised Unit Weight Error, Image Parameter Determination statistics, Non-Single Star solutions, and photometric blending as provided by Gaia, identifying hierarchical Ultracool triple systems. Our catalogue includes 17 White Dwarf - Ultracool Dwarf systems, whose ages are determined using cooling models. We also use the Gaia FLAME results and the BANYAN $\Sigma$ procedures to age 40 and 34 systems respectively, and derive mass estimates from evolutionary models.

==> DR3_obrital_solution_binaries.tex <==
 114832620743735808 & Gaia EDR3 114832620743735808 &	42.03952436 , 27.06811176	& \multirow{2}{*}{19.0576}  & \multirow{2}{*}{437.397864}	 &	43.57040024 &	K8 &	7.379911 &	6.791135 &	7.794708 &	6.06400013 & 5.690999985 & 5.614999771 \\

114832620743735040 & LP 354-414 & 	42.04194929, 27.07333447 & & & 43.44900131 & M5V & 13.911915 & 12.610563 & 15.72378 & 10.72799969 & 10.17399979 & 9.866000175 \\
\hline
144835853524677632 & LP 358-478 &69.72785619,21.79584643 & \multirow{2}{*}{14.1412} & \multirow{2}{*}{646.014823} & 21.57060051 & M5.5e & 16.046728 & 14.66189 & 18.299646\\

144835750444572416 &  Gaia EDR3 144835750444572416 & 69.72413844, 21.79749886 & & & 21.88990021 & & & & & & & \\
\hline

1021547495929308800 & Gaia EDR3 1021547495929308800 & 142.803457, 54.07053147 & \multirow{2}{*}{55.7951} & \multirow{2}{*}{7461.133352} & 7.478099823 & L5 & 14.092893	& 13.093988 & 15.104929 & 11.81700039 & 11.18700027 & 10.9829998\\

1021547457274626688 & SDSS J093110.53+540326.4 & 142.7933907, 54.05726467 & & &  7.823699951 & M7 &20.432755 &	18.957024 & 21.573341 &	16.125 &	15.91600037 &	15.41399956\\
\hline

644054092909736704 &  Gaia EDR3 644054092909736704 & 143.8655317, 22.55677674 & \multirow{2}{*}{758.026}	& \multirow{2}{*}{85234.08161} & 8.893461227	& & 13.58274 &	12.575141 & 14.605918& 11.26799965& 10.57499981 & 10.38099957\\

641048298702666752 & SDSS J093554.35+222205.4 & 143.9763323, 22.36813346 &&& 8.167784691 & M8V& 19.702856& 18.23171	&21.174803&	15.75300026&	15.12800026&	14.7670002\\
\hline

1527848102028547840 & MCC 677 &	192.6369145, 40.37116714&	\multirow{2}{*}{115.8955}&	\multirow{2}{*}{3856.228773} & 30.05410385 &M4	& 10.71255	& 9.737026&	11.682234&	8.505000114&	7.833000183&	7.631999969\\

1527847964589594624 & LP 217-82	& 192.6711526, 40.36047368	&&&		29.97580528&	M6&	16.512737&	15.078135&	19.15177&	12.75399971&	12.11200047&	11.77900028\\
\hline

1721485122019988608  & Gaia EDR3 1721485122019988608&	232.4646297, 82.26350843&	\multirow{2}{*}{68.78832}&	\multirow{2}{*}{4462.166917}&	15.41590023&	M1&	6.831625&	6.483267&	7.029218&	6.093999863&	5.927999973&	5.886000156\\

1721485122020033280 & 2MASS J15294565+8215328&	232.4424601,82.25901912&&&	16.02020073&	M5&	17.03678&	15.505441&	18.911379&	13.26799965&	12.73200035&	12.38199997\\
\hline

2562742595373569280 & HD 8291&	20.57818952,3.512414897	& \multirow{2}{*}{43.77025}&	\multirow{2}{*}{2298.652388}&	19.04170036&	M3&	8.458453&	7.963873&	8.778291&	7.418000221&	7.137000084&	7.070000172\\

2562743355583039616 & HIP 6407B&	20.57091921,3.522528046	&&&		19.75569916&	L1&	20.297554&	18.725279&	21.560135&	15.47099972&	14.65100002&	14.40200043\\
\hline

2665079816223169664 & ULAS J230818.73+062951.4&	347.0788978	, 6.498149489&	\multirow{2}{*}{3802.916644}&	\multirow{2}{*}{0.155455862}	& 24.46299934 &	M8 &	13.447574	& 12.267598	& 14.898524	&&& \\

2665079816222446080 & ULAS J230818.73+062951.4&	347.0781979,6.497344354	&&&		24.30500031&	L0&	18.0086&	16.3095&	20.17141& &&& 
\hline

3650384995128745472 & UCAC3 178-131495&	222.4151671,	-1.306562966&	\multirow{2}{*}{51.61619365}&\multirow{2}{*}{3782.625877}&	13.64559841&	M6&	11.692391&	10.722925&	12.653514&	9.524999619&	8.868000031&	8.67800045\\

1158372058624311552 & SDSS J144931.36+045531.4&	222.3936209,-1.293494649&&&			13.82567501&	M6&	18.564976&	17.06872&	20.605309&	14.64299965&	14.00500011&	13.60299969\\
\hline

6340820683358738944 &  Gaia EDR3 6340820683358738944&	224.3032417,	-1.272779358&	\multirow{2}{*}{1.34590429}&	\multirow{2}{*}{141.686069}&	9.499199867&	M0&	14.189117&	13.130664&	15.31855 &&&\\

6340820679064049536 & SDSS J145712.57-011620.2&	224.3022478,-1.272545968&&& 9.137599945&	M4&	17.4111&	16.0689&	19.0974&&&	\\
\hline

6361974428084996992 &  EDR3 6361974428084996992&	307.4446472,	-79.16935266&	\multirow{2}{*}{144.2618209}&	\multirow{2}{*}{7.170355814}&	20.11919975&	L1&	15.057488&	13.864156&	16.577234&	12.22599983&	11.6789999&	11.41800022\\

6361974496804484608 &  EDR3 6361974496804484608&	307.3950501,	-79.17033373	&&&		19.62599945&	L0&	20.549452&	18.954739&	21.265682&	15.55700016&	14.8210001&	14.54100037\\
\hline













==> LUWE.tex <==
HD 8291                       & 2.86 & 8.46  & 3.89             & 0.44              \\
\hline
Gaia EDR3 114832620743735808  & 2.05 & 7.38  & 2.43             & 0.07              \\
\hline
LP 358-478                    & 2.05 & 16.05 & 3.31             & 0.15              \\
\hline
UCAC3 178-131495              & 9.2  & 11.69 & 3.81             & 0.09              \\
\hline
Gaia EDR3 1721485122019988608 & 4.18 & 6.83  & 0.98             & 0.06              \\
\hline

==> WD_ages.tex <==

GD 280                         & 0.550 & 0.661  &  4.20  &  9490 &   7.93   \\
\hline
LP 554-15                      & 0.742 & 0.791  & 1.30  & 10400 & 8.22 \\
\hline
2MASS J00301179-3740483        & 0.565 & 1.34  & 4.58   & 7250  & 7.95 \\
\hline
Gaia EDR3 1438686535171582080* & 0.555 & 1.91  & 5.56   & 6280  & 7.94 \\
\hline
Gaia EDR3 1393854635743747200* & 0.651 & 2.29  & 3.38   & 6440  & 8.01 \\
\hline
SDSS J160555.83-200119.4*      & 0.521 & 4.74  & \textit{ 13.4} & 4980  & 7.90 \\
\hline
SDSS J120815.59+084543.0       & 0.504 & 4.85  & \textit{ 13.4} & 4900  & 7.87 \\
\hline
Gaia EDR3 5863122429179888000* & 0.473 & 6.31  & \textit{ 13.4}  & 4440  & 7.82 \\
\hline


==> WD_table.tex <==

GD 280  & DA & 16.88 & 12.25 &  WD & \multirow{2}{*}{1}\\
2MASS J01545796+4819596& M9 & 20.44 & 15.99&  HPM\\
\hline

LP 554-15 & DA & 17.57 & 12.40 & WD & \multirow{2}{*}{2}\\
SDSS J115948.20+070658.8  & M7 & 19.18 &14.20& LM \\
\hline

2MASS J00301179-3740483  & DA & 16.61 & 13.23 & WD & \multirow{2}{*}{3} \\
2MASS J00300625-3739483 & M9 & 19.85& 16.47 & BD \\



\hline

Gaia EDR3 1438686535171582080 & - & 19.33 & 13.75 & WD & \multirow{2}{*}{4}\\
SDSS J171036.96+621029.4  & M7 & 20.43 & 14.65&  LM \\ 
\hline

Gaia EDR3 1393854635743747200  & - & 19.78 & 13.87 & WD & \multirow{2}{*}{5}\\
2MASS J15110126+4442387  & M7V & 19.61 & 13.62 & LM\\



\hline

SDSS J160555.83-200119.4  & - & 18.95 & 14.75 & WD & \multirow{2}{*}{6}\\
2MASS J16055578-2001270  & M7V & 18.76 & 14.50 & HPM\\
\hline

SDSS J120815.59+084543.0 & DA & 18.07 & 14.79 & WD & \multirow{2}{*}{7}\\
2MASS J12081689+0845279 & M9V & 18.27 & 15.00 & LM\\


\hline

Gaia EDR3 5863122429179888000 & - & 19.58 & 15.19 & WD & \multirow{2}{*}{8}\\
2MASS J12564352-6202041 & L7 & 20.72 & 16.48 & BD\\

\hline




==> blended_close_binaries.tex <==
Gaia DR3 2542723688382428416 & \multirow{2}{*}{0.73} & 18.57& 1.82 & 42 & 42 \\

Gaia DR3 2542723688384558208 & & 19.32 & - & 0 & - \\
\hline
NSN 170A & \multirow{2}{*}{0.84} & 18.27 & 1.94 & 25 & 21 \\

NSN 170B & & 18.29 & 2.01 & 17 & 15 \\
\hline
Gaia DR3 3271777035211085312 & \multirow{2}{*}{0.75}& 17.26 & 1.82 & 58 & 58 \\

Gaia DR3 3271777035212786944 &  & 18.52 &  - & 0 & - \\
\hline
Gaia DR3 5563853506012603776 & \multirow{2}{*}{0.85} & 17.82
&2.23 & 26 & 26 \\

2MASS J06572547-4019134 & & 17.89 &  2.31 & 8 & 8 \\
\hline
SDSS J131711.51+184923.0 & \multirow{2}{*}{0.73} &   17.27 & 2.22 & 21 & 21 \\

Gaia DR3 3938910830669894016 & & 17.28 &  2.23 & 17 & 17 \\
\hline
2MASSI J1550084+145517A & \multirow{2}{*}{0.87} & 20.18 &2.00 & 54 & 54 \\

2MASSI J1550084+145517 & & 20.87 &  - & 54 & 54 \\
\hline
Gaia DR2 1372203812978252032 & \multirow{2}{*}{0.69} & 18.49 & 1.85 & 47 & 47 \\

Gaia DR3 1372203812978251904 & & 19.29 &  - & 0 & - \\
\hline
Gaia DR3 1361561227617464704 & \multirow{2}{*}{0.58} & 19.04 &2.20 & 24 & 24 \\

Gaia DR3 1361561227616589184 & & 19.15 &  2.31 & 4 & 4 \\
\hline
DENIS-PJ220002.05-303832.9A & \multirow{2}{*}{0.98} & 18.46 & 1.99 & 47 & 47 \\

DENIS-PJ220002.05-303832.9B & & 19.08 &  - & 0 & - \\
\hline
SDSS J223736.62+143459.6 & \multirow{2}{*}{0.58} & 19.09 & 2.10 & 16 & 16 \\

Gaia DR3 2732787501743069312 & & 19.33 &  - & 0 & -


==> blended_far_binaries.tex <==
Gaia EDR3 363570806968744960 & \multirow{2}{*}{17.5} & 1.19 & 28 & 1 \\

2MASS J01040814+3623016 &  & 1.96 & 28 & 28 \\
\hline
2MASS J02192210-3925225 & \multirow{2}{*}{3.90} & 1.40 & 72 & 3 \\

2MASS J02192210-3925225B &  & 1.82 & 7 & 0 \\ \cline{2-2}
\hline
LP 300-55 A & {\multirow{2}{*}{2.54}} & 1.37 & 28 & 2 \\

LP 300-55 B &  & 2.13 & 2 & 1 \\ 
\hline
LP 125-7 & \multirow{2}{*}{136.2} & 1.10 & 58 & 0 \\

LP 125-8 A &  & 2.13 & 50 & 50 \\
\hline
2MASS J10271395+5747027 & \multirow{2}{*}{1.25} & 1.63 & 44 & 15 \\

Gaia EDR3 854959561491166080 &  & 1.84 & 29 & 12 \\
\hline
G 199-16 & \multirow{2}{*}{3.03} & 1.18 & 50 & 17 \\

Gaia EDR3 1583484215025634688 &  & 1.81 & 5 & 5 \\
\hline
Gaia EDR3 3705763723623026304 & \multirow{2}{*}{2.15} & 1.11 & 65 & 1 \\

ULAS J125015.55+045506.6 &  & 2.19 & 50 & 1 \\
\hline
Gaia EDR3 4426055818208228352 & \multirow{2}{*}{341.2} & 1.79 & 42 & 42 \\

SDSS J155423.52+041410.1 &  & 1.40 & 45 & 2


==> coefficents.tex <==
$a_0$ & 10.9 \\
$a_1$ &  -32.7 \\
$a_2$ &  \num{1.07e2} \\  
$a_3$ &  \num{-2.66e2} \\ 
$a_4$ &  \num{6.87e2} \\ 
$a_5$ &  \num{-11.9e2} \\
$a_6$ &  \num{11.3e2} \\ 
$a_7$ &  \num{-5.25e2} \\ 
$a_8$ &   95.3\\ 
b &  0.664 \\ 
\hline
